The survival of scientific stylization

This study elaborates a text-based metric to quantify the unique position of stylized scientific research, characterized by its innovative integration of diverse knowledge components and potential to pivot established scientific paradigms. Our analysis reveals a concerning decline in stylized research, highlighted by its comparative undervaluation in terms of citation counts and protracted peer-review duration. Despite facing these challenges, the disruptive potential of stylized research remains robust, consistently introducing groundbreaking questions and theories. This paper posits that substantive reforms are necessary to incentivize and recognize the value of stylized research, including optimizations to the peer-review process and the criteria for evaluating scientific impact. Embracing these changes may be imperative to halt the downturn in stylized research and ensure enduring scholarly exploration in endless frontiers.

==> tab_c5_c10_sbs_lag.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{4}{c}}
\toprule
                                             &\multicolumn{1}{c}{\shortstack{C$\textsubscript{5}$ }}&\multicolumn{1}{c}{\shortstack{C$\textsubscript{10}$ }}&\multicolumn{1}{c}{\shortstack{Sleeping beauty strength }}&\multicolumn{1}{c}{\shortstack{Turnaround time }}\\\cmidrule(lr){2-2}\cmidrule(lr){3-3}\cmidrule(lr){4-4}\cmidrule(lr){5-5}
                                             &\multicolumn{1}{c}{(1)}   &\multicolumn{1}{c}{(2)}   &\multicolumn{1}{c}{(3)}   &\multicolumn{1}{c}{(4)}   \\
\midrule
Stylization                                  &        -3.0591***&        -2.9435***&         3.5275***&        20.1456***\\
                                             &       (0.0079)   &       (0.0086)   &       (0.1225)   &       (0.5435)   \\
Team size                                    &         0.0020***&         0.0020***&        -0.0556***&         0.1077***\\
                                             &       (0.0002)   &       (0.0002)   &       (0.0035)   &       (0.0079)   \\
Field size                                   &        -0.0000***&        -0.0000***&         0.0001***&         0.0000***\\
                                             &       (0.0000)   &       (0.0000)   &       (0.0000)   &       (0.0000)   \\
Reference count                              &         0.0057***&         0.0059***&        -0.0020***&        -0.0106***\\
                                             &       (0.0000)   &       (0.0000)   &       (0.0004)   &       (0.0013)   \\
Average knowledge age                        &        -0.0644***&        -0.0597***&         0.0968***&         3.7105***\\
                                             &       (0.0001)   &       (0.0001)   &       (0.0017)   &       (0.0183)   \\
Average career experience                    &         0.0106***&         0.0108***&         0.0526***&        -0.3954***\\
                                             &       (0.0001)   &       (0.0001)   &       (0.0018)   &       (0.0068)   \\
Knowledge age dispersion                     &         0.0261***&         0.0294***&         0.1265***&        -2.4682***\\
                                             &       (0.0001)   &       (0.0001)   &       (0.0018)   &       (0.0168)   \\
Career experience dispersion                 &         0.0089***&         0.0086***&        -0.0189***&         0.0889***\\
                                             &       (0.0001)   &       (0.0001)   &       (0.0017)   &       (0.0073)   \\
Year FE                                      &            Yes   &            Yes   &            Yes   &            Yes   \\
Field FE                                     &            Yes   &            Yes   &            Yes   &            Yes   \\
\midrule
{\( N \)}                                    &       25182058   &       25182058   &        5750318   &        5751006   \\
{(Pseudo) \( R^2 \)}                         &           0.25   &           0.24   &           0.03   &           0.05   \\
\bottomrule
\end{tabular}
}

